PANEM: A Heuristic Latency Model

Accurate pre-silicon memory modeling is essential for achieving meaningful representation of workloads on cloud-class many-core processors. Existing options force a poor tradeoff between fidelity and speed: fixed-latency models are fast but misleading, while cycle-accurate DRAM models are costly and difficult to scale across large study spaces or onto single-core environments. This paper presents PANEM, a lightweight event-driven heuristic model that has guided four generations of commercial server-core development at Ampere Computing. PANEM converts bandwidth-latency characterization data into a dynamic request-bytes/latency response, allowing miss latency to adapt to transient demand, queuing pressure, and read/write mix during simulation. Integrated into a single-core flow with configurable system-loading assumptions, PANEM enables realistic bandwidth constraints and contention-aware latency behavior without sacrificing throughput. Across a broad cloud workload trace suite, PANEM avoids the optimistic and pessimistic biases of fixed-latency baselines, yields more reliable conclusions for prefetching and dynamic throttling studies, and materially improves core-resource sizing decisions. These results show that a calibrated, contention-aware abstraction can deliver practical predictive value for industrial design-space exploration at simulation costs similar to fixed-latency models.

==> font/test.tex <==
hello world
